BATS: Best Action Trajectory Stitching

The problem of offline reinforcement learning focuses on learning a good policy from a log of environment interactions. Past efforts for developing algorithms in this area have revolved around introducing constraints to online reinforcement learning algorithms to ensure the actions of the learned policy are constrained to the logged data. In this work, we explore an alternative approach by planning on the fixed dataset directly. Specifically, we introduce an algorithm which forms a tabular Markov Decision Process (MDP) over the logged data by adding new transitions to the dataset. We do this by using learned dynamics models to plan short trajectories between states. Since exact value iteration can be performed on this constructed MDP, it becomes easy to identify which trajectories are advantageous to add to the MDP. Crucially, since most transitions in this MDP come from the logged data, trajectories from the MDP can be rolled out for long periods with confidence. We prove that this property allows one to make upper and lower bounds on the value function up to appropriate distance metrics. Finally, we demonstrate empirically how algorithms that uniformly constrain the learned policy to the entire dataset can result in unwanted behavior, and we show an example in which simply behavior cloning the optimal policy of the MDP created by our algorithm avoids this problem.

==> checklist.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section*{Checklist}

%%% BEGIN INSTRUCTIONS %%%
The checklist follows the references.  Please
read the checklist guidelines carefully for information on how to answer these
questions.  For each question, change the default \answerTODO{} to \answerYes{},
\answerNo{}, or \answerNA{}.  You are strongly encouraged to include a {\bf
justification to your answer}, either by referencing the appropriate section of
your paper or providing a brief inline description.  For example:
\begin{itemize}
  \item Did you include the license to the code and datasets? \answerYes{See Section~\ref{gen_inst}.}
  \item Did you include the license to the code and datasets? \answerNo{The code and the data are proprietary.}
  \item Did you include the license to the code and datasets? \answerNA{}
\end{itemize}
Please do not modify the questions and only use the provided macros for your
answers.  Note that the Checklist section does not count towards the page
limit.  In your paper, please delete this instructions block and only keep the
Checklist section heading above along with the questions/answers below.
%%% END INSTRUCTIONS %%%

\begin{enumerate}

\item For all authors...
\begin{enumerate}
  \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \answerYes{}
  \item Did you describe the limitations of your work?
    \answerYes{In Section \ref{sec:experiments} we discuss observed limitations of our algorithm}
  \item Did you discuss any potential negative societal impacts of your work?
    \answerNo{We do not see potential negative societal impacts of a conservative offline RL algorithm.}
  \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
    \answerYes{We believe offline RL is a prosocial field as it allows for RL agents to be trained more safely than in the online setting.}
\end{enumerate}

\item If you are including theoretical results...
\begin{enumerate}
  \item Did you state the full set of assumptions of all theoretical results?
    \answerYes{In Section \ref{ss:extendo} we give a full set of assumptions for our theoretical work.}
	\item Did you include complete proofs of all theoretical results?
    \answerYes{Theorem \ref{thm:bisimulation} has a proof in the appendix and Corollary \ref{cor:policy_improvement} is an immediate consequence of the theorem.}
\end{enumerate}

\item If you ran experiments...
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
    \answerYes{We include our code in the supplemental along with instructions, and we plan to release our code online at a later date.}
  \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
    \answerYes{We specify this in sections \ref{sec:experiments} and \ref{app:hyperparameters}. }
	\item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
    \answerYes{We report standard errors for all experiments we ran with quantitative evaluation.}
	\item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
    \answerYes{We discuss this in section \ref{sec:experiments}}
\end{enumerate}

\item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
\begin{enumerate}
  \item If your work uses existing assets, did you cite the creators?
    \answerYes{We make heavy use of D4RL and cite them.}
  \item Did you mention the license of the assets?
    \answerNA{}
  \item Did you include any new assets either in the supplemental material or as a URL?
    \answerNA{}
  \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
    \answerNA{}
  \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
    \answerNA{}
\end{enumerate}

\item If you used crowdsourcing or conducted research with human subjects...
\begin{enumerate}
  \item Did you include the full text of instructions given to participants and screenshots, if applicable?
    \answerNA{}
  \item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
    \answerNA{}
  \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
    \answerNA{}
\end{enumerate}

\end{enumerate}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


==> futurework.tex <==
NOT USED

\section{Future Work}
We leave to future work several exciting problems. First, we'd like to extend the setup and theory to a probabilistic setting. This will allow us to address a more realistic setting and better understand our algorithm's properties.
Second, we'd like to extend our algorithm to propose places where samples can be taken from a generative version of the MDP as in \cite{azar_generative}. We believe that there is possibly analysis doable on the graphical reduced MDP that would allow us to get a very sharp picture of what stitches would be best to try to make with a small sampling budget. We'd also like to extend the theory to give concrete dependencies on modeling error and error in computing the bisimulation metric for our value function bounds. We look forward to addressing these exciting questions!

==> intro_adam.tex <==
\section{abstract}
In Offline Reinforcement Learning, we attempt to learn an effective control policy from a pre-collected set of logged environment interactions. From this offline dataset, we want to learn a policy that is superior to the behavioral policy that collected the data. However, it can be difficult to learn a policy that acts differently than the behavioral policy, and yet maintains a state-action distribution that is in the support of the behavioral dataset where the models can be effective. Prior approaches, have addressed this issue by incorporating conservatism in their learned models of the policy, dynamics, or Q-function. In this work, we instead focus on constructing a limited finite MDP based off of short horizon stitching of the disjoint trajectories available in the dataset. Within this better connected finite MDP, we perform value iteration to recover the MDP's optimal policy. By behavior cloning this policy, we can learn a policy that improves by connecting good behaviors available in the dataset. Additionally, we show how we can upper and lower-bound the true value function using our finite MDP.


\section{Introduction}
RL has recently made large strides in TODO: strides. In its standard formulation, RL requires online environment interactions collected continually by an evolving exploratory policy. Following this formulation, many of the most impressive recent deep RL results often require orders of millions to billions of online samples to learn effective policies. Thus, it is unsurprising that many of these successes have been limited to simulated or well-controlled laboratory settings, where it is relatively easy to collect large amounts of online samples. However, there has been limited success in translating these approaches to many real-world applications such as automated driving or robot-assisted surgery, due to the inherent dangers and costs in collecting online exploratory data with an unreliable policy.

In order to alleviate the need for exploratory online data collection, many recent works have shifted to exploring the offline RL paradigm. In offline RL, we assume we have access to a fixed dataset of pre-collected environment interactions, and with this limited dataset we attempt to learn a policy that will be effective immediately at deployment. However, naively applying many of the SOTA online RL algorithms leads to dismal results. In particular, these algorithms suffer from a dangerous combination of distribution shift and model exploitation.

When states and actions are continuous, the major primitives used in RL are dynamics models which predict future states from current states and actions, value function estimators which predict the state value ($V(s)$), state-action value ($Q(s, a)$), or advantage ($A(s, a)$), and parameterized policies which sample actions given a state. The major paradigms of reinforcement learning apply these pieces to learn a controller: actor-critic methods alternatingly train a policy (actor) and state-action value function estimate (critic), and model-based RL methods run a planning algorithm over dynamics models. These methods all rely on recursive approximations, which appear under a variety of names as a classic problem with reinforcement learning algorithms. 

For actor-critic methods, the recursive bellman updates inevitably introduce errors due to the distribution shift between the learned policy and the behavioral policy. Then, the policy optimistically exploits these model errors in the Q-function, which often leads to a self-reinforcing cycle that causes the Q-values to diverge. In dynamics model-based methods, the combination of small initial errors and test-time distribution shift often leads to ever accumulating model-error. While distribution shift and model exploitation are potential issues in Online RL, these problems are more severe in the offline setting as the agent cannot collect additional experience to rectify consistent errors in estimation or planning.

In order to mitigate these issues, recent prior work in Offline RL have explored incorporating many different types of conservatism in the optimization process. These approaches can be broadly grouped into three sets of approaches based on the type of conservatism they incorporate.

The first set of approaches use actor-critic methods \citep{brac,bear}, but incorporate policy constraints to limit the difference between the learned policy and the behavioral policy that collected the data in order to mitigate distribution shift. The second set of approaches use MB RL\citep{mopo,morel}, but leverage uncertainty-aware dynamics models to deter the policy from taking action with high model uncertainty. The third set of approaches add conservatism directly to the Q-function \citep{cql} in order to directly discourage the policy from extrapolating optimistically. Rather than incorporating conservatism directly into one of the previously described RL primitives like these approaches, BATS acts conservative by restricting the policy optimization to a severely constrained MDP.

Specifically, BATS introduces a new primitive through a novel and conservative way of looking at the replay buffer. Building off the idea that a dataset of trajectories is finite, we treat this MDP itself as a primitive in our algorithm. We add advantageous transitions between separate trajectories with a short-horizon planning algorithm using a dynamics model and maintain upper and lower bound estimates on the value of the policy. In this work, we give a construction of this MDP, theoretically justify our derived value function estimates, and investigate its properties. We also propose and evaluate an offline RL algorithm that naturally follows from the construction. Our algorithm has competitive performance on many baselines, and often performs better when the offline data is goal-agnostic.


==> intro_viraj.tex <==
\section{Introduction}
Reinforcement Learning (RL) has recently made large strides in TODO: strides.
However, in its standard formulation RL requires an untrained policy to interact with the environment, often for large numbers of trials, in order to produce a trained policy.
In many applications, large amounts of potentially unsafe operation is infeasible but datasets of logged environmental interactions are available.
In the setting we consider here, \emph{offline reinforcement learning} \citep{levine2020offline}, a policy is synthesized with access only to the dataset and then only executed in the real environment when being evaluated after training is complete.

When states and actions are continuous, the major primitives used in RL are dynamics models which predict future states from current states and actions,
value function estimators which predict the state value ($V(s)$), state-action value ($Q(s, a)$), or advantage ($A(s, a)$), and parameterized policies which sample actions given a state. The major paradigms of reinforcement learning apply these pieces to learn a controller:
actor-critic methods alternatingly train a policy (actor) and state-action value function estimate (critic),
model-based RL methods run a planning algorithm over dynamics models,
and weighted behavior cloning regresses a policy onto observed actions typically weighted by some function of a value function estimate.
These methods all rely on recursive approximations, which appear under a variety of names as a classic problem with reinforcement learning algorithms. In particular, the following three problems all appear in the previous methods, which are related by this failure case:
\begin{itemize}
    \item Deep value function learning through recursive TD updates minimizing $\left( Q^\pi_\theta(s, a) - \left(r(s, a) + Q^\pi_\theta(s', \pi(s')\right)\right)^2$ can be subject to instability due to small optimistic errors exploding over many iterations.
    \item Small initial errors in long-horizon dynamics model planning can become large errors after many timesteps.
    \item In long trajectories of actions leading to high reward, it is difficult to assign credit to decisions for which counterfactual actions would have resulted in much worse returns.
\end{itemize}
In the offline setting, these problems are more severe, as the agent cannot collect further experience in order to rectify consistent errors in estimation or planning.
BATS introduces a new primitive through a novel way of looking at the replay buffer. Building off the idea that a dataset of trajectories is a finite MDP, we treat this MDP itself as a primitive in our algorithm. We add advantageous transitions with a short-horizon planning algorithm using a dynamics model and maintain upper and lower bound estimates on the value of the policy. Though computationally expensive in its most naive form, our algorithm leverages the rich information available about a finite MDP to avoid naively planning between all pairs. In this work, we give a construction of this MDP, theoretically justify our derived value function estimates, and empirically investigate its performance and scaling as well as the gaps between our theory and practice. Our algorithm has state-of-the-art performance on low-dimensional maze problems and is competitive with leading algorithms on high-dimensional simulated robotics tasks.

==> midpoint_method.tex <==
\subsection{Viraj Mid Point Report Text}
I propose Best-Action Trajectory Stitching (BATS), a method which takes the good characteristics of the preceding methods while enforcing provable stability in training. If we assume for now a deterministic MDP and a dataset which consists of trajectories which were rolled out in the MDP (as opposed to disjoint transitions), we can describe the dataset by a graph with nodes representing each state seen in the graph and edges labeled with the action which connects two states and the reward obtained for doing so. This graph is itself a tabular MDP, albeit a very boring one. Running value iteration on the graph would give each state the value of the observed return from that state.

Since each node represents a state, we can compute a new graph consisting of the same nodes and edges consisting of all the pairs of nodes of which the states are less than $\epsilon$ apart. We can also train an ensemble of dynamics models over our dataset. Then, for each pair of states which are neighbors in our neighbors graph, we can use our dynamics model plan transitions from their predecessor states to the opposite neighbors, thereby stitching the two trajectories. This can be made robust by for example using CEM to find the action that minimizes the 80th percentile distance from the target state predicted by our ensemble and only accepting the stitch if it is within $\delta$ of the goal.

At this point we now have a much more interesting and hopefully networked MDP, which should have many connections between the trajectories. We can then run value iterations to convergence over the (finite) MDP, which must converge in polynomial time to the true value functions. Finally, we can run behavior cloning over the optimal actions in our new graph.

This algorithm avoids the issues of value function blowup, stays well in the support of our data, and allows for good actions from different trajectories to be incorporated into a final policy.

There are two major theoretical questions: if the model has a particular validation error and we are asking to plan the action to within $\delta$ accuracy of the target state, how much error will be induced in the value function by assuming an edge which satisfies these criteria ends up in the same state. Ideally, this would be in the form of a lower bound on the true value function $V^\pi \geq \hat{V}^\pi - C(s, a)$. Second, it would be great to give a bound on the optimal value function of the form $V^*(s) \leq \hat{V}^\pi(s) + C(G)$. This would tightly characterize the theoretical performance of the algorithm and allow us to think confidently about deploying a policy in the real world after learning with offline data.

==> old_method.tex <==
\begin{figure}[ht]
     \centering
     \includegraphics[width=\textwidth]{NeurIPS2021/figures/cartoon.pdf}
     %\caption{}
     \label{fig:stitch_cartoon}
    \caption{\textbf{A Cartoon of the Core Idea of BATS.} The left panel shows the MDP formed by the logged dataset and the right panel shows the MDP after running BATS. At first, the start state displayed has low value; however, after planning trajectories (dashed blue lines) between states and running value iteration, the start state achieves high value.}
    \label{fig:cartoon}
\end{figure}

\section{Method}
% from Jeff: add a sketch of a graph that explains the point
% maybe just make a bulleted list that RL always fails because of:
% - value function estimation blowup
% - compounding errors in long horizon planning
% - issues with credit assignment in long horizon sequential decision making
% from Jeff re: brittleness to hyperparameters and compute requirements -- put this in the future work
% The insight that our work builds upon is that the logged data itself is a tabular MDP. That being said, it is an extremely uninteresting MDP in which, for every state, there is only one possible action that an agent can take. 

In this section we describe our algorithm: Best Action Trajectory Stitching (BATS). Our method builds on the core idea that the offline dataset itself is a tabular MDP, where the states of the MDP are the states encountered by the behavioral policy, and the actions are those taken by the policy. Having a tabular version of the MDP in question would be ideal since one can perform value iteration exactly and avoid the instabilities caused from the deadly triad \citep{deadly_triad}. Furthermore, assuming transitions in such a tabular MDP were correct, one could easily trace out where in state space a sequence of actions leads. The resulting MDP could then be leveraged to learn a continuous policy which could operate on the real environment.

However, the logged data without modification is an extremely uninteresting MDP since for each state there is at most one action that can be taken (the same one taken by the behavioral policy). BATS makes this MDP more interesting by planning trajectories--or ``stitches''--between states using a learned dynamics model. To ensure that the stitches from our model are feasible, we limit the number of actions that can be taken to stitch two states. Because there are on the order of $n^2$ different stitches that can be made, our algorithm prioritizes making stitches with high positive advantage in regions that an optimal policy would visit. In the next subsection, we describe these details in more depth.

% We now introduce the BATS Algorithm.
% Idea is built off of the key idea that logged dataset itself is an MDP
% Dealing with a tab MDP would be better for us bc has many freedoms such as value iteration
% Can better reason about what optimal trajectories will look like
% At end of day we can use some form of imitation learning to create policy for the environment.

% This MDP can be made better by stitching.
% This should be ok because small rollouts are trustworthy
% Since there are so many possibilities we focus on places with high advantage.
% We describe the


% 
% This tabular MDP setting gives us additional freedoms like 


% The BATS algorithm is best explained from a posture of extreme conservatism. We choose to primarily trust two available components: the actual transitions available in the dataset and short-horizon transitions from a dynamics model with high confidence in the support of our data. We will give an intuitive formulation of the algorithm here and subsequently formalize it and prove theoretical properties.
% % \adamcomment{The use of primitives here seems to conflict with how you describe it in the intro.}\virajcomment{fair point I'll fix it}

% The BATS algorithm starts with a finite deterministic MDP derived from the dataset: it contains every state in the dataset and at each state the only actions available are the ones that were taken at that state in the dataset. 
% Any finite deterministic MDP can be represented by a graph with a vertex for each state and edges representing the actions allowing us to transition from one state to another.
% This graph must look like a set of mostly-disjoint components which each correspond to a trajectory. We can find the optimal value function for a finite MDP in polynomial time via value iteration \citep{Sutton1998}.
% This process avoids the traditional deadly triad of function approximation, bootstrapping, and off-policy learning, and thus is not subject to the problem of value function blowup\citep{deadly_triad}.
% A natural idea would be to then learn via supervised behavior cloning a parameterized policy over our finite MDP which takes the optimal action available at each state but extends to the continuous real problem. 
% Performing value iteration and cloning as discussed using only the dataset for our finite MDP reduces to behavior cloning in the case where all trajectories are disjoint and is slightly better than behavior cloning (as only the higher-value actions would be taken) in the case where trajectories overlap.

% \begin{figure}
%     \centering
%     \begin{subfigure}[b]{0.4\textwidth}
%          \centering
%          \includegraphics[width=\textwidth]{NeurIPS2021/figures/stitching.pdf}
%          %\caption{$y=x$}
%          \label{fig:y equals x}
%      \end{subfigure}
%     \begin{subfigure}[b]{0.4\textwidth}
%          \centering
%          \includegraphics[width=\textwidth]{NeurIPS2021/figures/maze2d-umaze-v1_graph.png}
%          %\caption{}
%          \label{fig:y equals x}
%      \end{subfigure}
%     \caption{Trajectories are stitched together with MDP edges to add potentially better actions to our approximate MDP. Here, state $s$ is being stitched to state $s'$ via action $a$ which gets reward $r$ (red dashed arrow). This will happen if $s$ and the predecessor state to $s'$ are nearest neighbors (blue dotted line).}
%     \label{fig:graphs}
% \end{figure}

% \color{green}[Jeff comments: The following paragraph seems to mix the concept of stitching and the mechanism to do so efficiently.  I would separate them.  First describe the concept and use an illustration of it.  Then second, or maybe even defer to the detailed implementation, describe how to find these stitches efficiently]
% \color{black}\virajcomment{I've attempted to fix this by cutting the details of how stitching happens to later, could also uncomment that paragraph below.}

% It is conceivable that in some states in the dataset there exists an alternative sequence of up to $k$ actions that would transition the agent back into another state in the dataset.
% In this case, we could add an edge or sequence of vertices and edges to the graph linking the two states. 
% If the states in the original MDP have a reasonable metric associated with them, we can leverage it to filter out reasonable transitions between states in the dataset. 
% In a dataset of $n$ MDP transitions, there are naively $n^2$ possible transitions between states to check for. This `check' takes the form of attempting to plan up to $k$ actions which arrive at the goal state. 
% For millions of examples this would result in trillions of planning problems which is computationally infeasible. 
% We address this issue by sampling from the occupancy distribution in our reduced MDP and attempting to plan new transitions by a heuristic of walking between $1$ and $k$ edges in our reduced MDP and one edge on a nearest-neighbor graph in the metric space on states. This gives edges for which there is a good initialization for the planning problem of the $k$ actions in the MDP edges.


% By repeatedly iterating the interleaved process of sampling from the occupancy distribution and walking to find edges, adding edge,s and solving the MDP before behavior cloning, we can add better and better actions which interpolate the dataset. Ultimately this results in a cloned policy which will outperform behavior cloning in a way which is easy to quantify given the information available in our finite MDP.

% viraj: this is the extra block explaining stitching -- took it out as it seems too detailed for this point. May add again later.
% This process takes two steps. First, we define an alternate set of edges between vertices of which the associated states are nearest neighbors according to the metric. 
%  Next, we sample a state from the occupancy distribution of our discrete MDP and assume as the universe of potential outgoing new transitions the states which can be reached by walking in some order exactly $1$ nearest-neighbor edge and up to $k$ discrete MDP edges from our sampled state. 
% For states in the universe of possible transitions, we compute the advantage of such a transition. If it is positive and the new transition would therefore improve our policy, we attempt to plan such a transition via search over our dynamics model initialized at the actions associated with the MDP edges encountered in our walk to the goal state.
% If the planning is successful according to our metric in getting within a tolerance $\epsilon$ of the goal state with high confidence, then the edge is added to the graph with the planned actions and a penalized reward that accounts for the planning error. 




% This setting is typical of standard benchmark tasks in simulation and is a fairly good model for systems with small noise. We leave to future work a probabilistic development of this algorithm, likely using some notion of KDE over our graph to analyze the algorithm behavior.




\subsection{The BATS Algorithm}
\label{sec:bats_algo}
Let $M$ be an MDP, $D$ be a dataset as in Section \ref{ss:preliminaries}, and $d(\cdot, \cdot)$ a metric over $\Statespace$. 
If we let $\hat{\Statespace}^{(0)} = \{s_i\}_{i\in[n]}$, $\hat{\Actionspace}_{i}^{(0)} = \{a_{i}\}_{i\in[n]}$, and $\hat{p}_0(s)$ be a discrete uniform distribution over all start states appearing in $D$, we can construct a finite MDP $\hat{M}_0 = \langle \hat{\Statespace}^{(0)}, \hat{\Actionspace}_{j}^{(0)}, \gamma, \hat{T}_0 = T, r_0, \hat{p}_0(s)\rangle$. 
We assume a trained dynamics model $T'$ with access to uncertainty estimates and a learned reward function. 
In our case, we use a probabilistic ensemble of neural network dynamics models as in \citet{PETS}.
We also compute a nearest neighbors graph over our states where there are edges between $s_i$ and $s_j$ if $d(s_i, s_j) < \delta$. We proceed by repeating in sequence the following steps starting from $i=0$ for as long as compute is available.

First, we perform value iteration on $\hat{M}_{i}$, giving an optimal policy $\pi_i$ and value function $\hat{V}_i$. Next, we sample a batch of states from the occupancy distribution $\{s_j\}_{j=0}^m \sim \mu_\gamma(s \mid \pi_i, \hat{p}_0)$. For each state $s_j$ in our sample, we consider all states $s'$ that are at most $k$ transitions in $\hat{M}_i$ away, exactly one nearest-neighbor transition away, and would be advantageous to stitch to such that $\hat{V}_i(s') > \hat{V}_i(\hat{T}_i(s_j, \pi(s_j)))$ and $s' \in \hat{\Statespace}^{(0)}$. Here, the intuition is that the actions taken to get to a neighboring state might be close to those that would get to $s'$. If adding a stitch to $s'$ would improve the current policy, than that stitch is worth adding.

Next, for all possible stitches $(s_j, s')$ found, we plan with our dynamics model using the cross-entropy method (CEM) as in \citet{PETS} for $\ell = 1, \dots, k$ to find $\argmin_{a_0, \dots, a_{\ell-1}}d(s', \hat{s}_{\ell})$ s.t $\hat{s}_{t+1} = T'(\hat{s}_t, \hat{a}_t), \hat{s}_0 = s_j$. If the distance is less than $\epsilon$, we add the transition to our graph.
% This involves adding dummy states $s_1,\dots, s_{k-1}$ to $\hat{\Statespace}^{(i + 1)}$ for intermediate steps in the planned actions, adding $a_1$ to $\hat{\Actionspace}_{j}^{(i + 1)}$ and for each of our dummy states similarly adding as the only available action the one from our plan.
This involves adding states $\hat{s}_1,\dots, \hat{s}_{\ell-1}$ to $\hat{\Statespace}^{(i + 1)}$ and adding relevant transitions. Note that we prevent our algorithm from stitching to added states during future iterations.
% We then set $\hat{T}_{i + 1}$ such that $\hat{T}_{i + 1}(\hat{T}_{i + 1}(\dots \hat{T}_{i+ 1}(s_j, a_1), a_2),\dots, a_k)) = s'$. 
We penalize the reward associated with the added transition to $s'$ in our new MDP by letting $r_i(\hat{s}_{\ell-1}, s') = r(\hat{s}_{\ell-1}, \hat{a}_{\ell-1}) - \gamma d(s', \hat{s}_{\ell})$. 
Then after doing this for each stitch where planning was successful, our new MDP can be written as $\hat{M}_{i + 1} = \langle \hat{\Statespace}^{(i + 1)}, \hat{\Actionspace}_{j}^{(i + 1)}, \gamma, \hat{T}_{i + 1}, r_{i + 1},\hat{p}_0(s)\rangle$. From here, we can repeat the process, iteratively improving our policy. The algorithm terminates when no stitches with positive advantage can be found or the computational limit is reached.

After the algorithm completes, value iteration gives a policy $\pi$ which is optimal for our created MDP $\hat{M}_{n}$, but is unable to be applied on the true, continuous environment as it is only defined over $\hat{\Statespace}^{(n)}$. To remedy this, we first form a dataset of optimal trajectories from the MDP. For each start state, we use $\pi$ to choose which transitions to make and add the resulting path through the MDP to our dataset. For this work, we choose to learn our final policy by simply performing behavior cloning over this dataset. In general, though, any policy learning algorithm could be used to go from $\hat{M}_n$ to a policy over $\Statespace$.

% When the stitching iterations are finished (either after a finite number of iterations, which we use in practice, or when no stitches can be found which would improve the optimal policy on the reduced MDP), we simply generate data by rolling out the optimal reduced policy in the finite MDP.\virajcomment{TODO (Ian): explain the selection strategy we use}\ianx{I vote to put this whole paragraph in the experiment section because it is more details about how we conducted those specific experiments. Also I would vote not having behavior cloning be included in the BATS algorithm.}
% Then, we simply behavior clone a neural network policy on the dataset of optimal actions. This is the policy output by BATS. A pseudocode description of the process is given in Algorithm \ref{algo:bats}, where $\getNeighbors$ and VI are the nearest-neighbors operations and value iteration respectively. Further subroutines are given in Section \ref{s:subroutines}.

\paragraph{Hyperparameters}
Our algorithm has a number of hyperparameters of interest. Dynamics model training, metric learning, behavior cloning, and CEM all have parameters which trade off computation and performance. However, these are well-known methods which operate independently and for which hyperparameters selection is a relatively well-understood problem. The BATS algorithm itself requires a tolerance for value iteration, $\delta$ for the neighbors graph, $\epsilon$ for deciding whether to add stitches, a batch size $m$, a max number $k$ of actions in a stitch, and the number of iterations $n$. We further discuss how we determined hyperparameters for our experiments in the Appendix~\ref{app:hyperparameters}.


% Besides $\epsilon$, all of these should be set as large as fit in the memory and computational budget. $\epsilon$ can be determined by 1-dimensional grid search.
\begin{algorithm}
\caption{The BATS Algorithm}
\label{algo:bats}
\begin{algorithmic}
\Procedure{BATS}{$\{(s_{i}, a_{i}, s'_{i}, r_{i})\}_{i=1}^N$ trajectories, $k$, $n$, $m$ $\epsilon$, $\delta$, $\gamma$}
\State $\hat{M}_0 = \langle \bigcup_{i, t}(\{s_{it}\}\cup\{s'_{it}\}), \Actionspace_{s_{it}} =
\{a_i\},\gamma, T(s_{it}, a_{it}) = s'_{it}, R(s_{it}, a_{it}) = r_{it}, U(\{s_{i0}\}_{i=1}^N)\rangle$

\For{$i \in [n]$}
    \State $\hat{V}_i^*(\cdot), \pi_i(\cdot) \gets VI(\hat{M}_i)$
    \State neighbors $\gets \getNeighbors(\Statespace, \pi, \hat{M}_i, \delta)$
    \State $E' \gets []$
    \For{$j=1:m$}
        \State $s \sim \mu_{\hat{M}_i}(s \mid \pi_i)$
        \State $E \gets \getPotentialEdges(s, s, \hat{M}_i, \text{neighbors}, j)$
        \ForAll{$e \in E$}
            \State actions = $\testEdge(e, k, \epsilon)$
            \ForAll{action $\in$ actions}
                \State $E'$ += action
            \EndFor
        \EndFor
    \EndFor
    
    \State $\hat{M}_{i + 1} \gets \hat{M}_i \cup E'$
\EndFor

\State $V(\cdot), \pi(\cdot) \gets VI(\hat{M}_n)$

\Return $\hat{M}_n$
\EndProcedure

\end{algorithmic}

\end{algorithm}


